A Survey of Vision-Language Pre-Trained Models

As transformer evolves, pre-trained models have advanced at a breakneck pace in recent years. They have dominated the mainstream techniques in natural language processing (NLP) and computer vision (CV). How to adapt pre-training to the field of Vision-and-Language (V-L) learning and improve downstream task performance becomes a focus of multimodal learning. In this paper, we review the recent progress in Vision-Language Pre-Trained Models (VL-PTMs). As the core content, we first briefly introduce several ways to encode raw images and texts to single-modal embeddings before pre-training. Then, we dive into the mainstream architectures of VL-PTMs in modeling the interaction between text and image representations. We further present widely-used pre-training tasks, and then we introduce some common downstream tasks. We finally conclude this paper and present some promising research directions. Our survey aims to provide researchers with synthesis and pointer to related research.

==> sec-ack.tex <==
\section*{Acknowledgments}



==> sec-background.tex <==
\section{Background}\label{background}

In recent years, Transformer~\cite{vaswani2017attention} has gained great success in various areas, especially in natural language processing. Transformer-based models are able to draw global dependencies, which proves to be very effective in NLP tasks. The residual connection in Transformer layers makes it possible for transformer-based models to be bigger and deeper.

With the advance of transformer architecture and the increasing of computation power, pre-training and fine-tuning has become the paradigm to do NLP tasks. It has been proven that pre-training on large datasets helps the model learn universal representations, which could improve the performance on downstream tasks. Large Pre-trained Language Models~(PLM) such as BERT~\cite{devlin2018bert} and GPT~\cite{radford2018improving} have achieved state-of-the-art results on many downstream tasks. As for the field of CV, there are several breakthroughs in pre-trained models for vision tasks such as BEiT~\cite{bao2021beit} and MAE~\cite{he2021masked}.

Due to the success of pre-training methods in the field of CV and NLP, many have tried to apply the same strategy to V-L tasks. Intuitively, pre-training on a large image-text dataset can help V-L models learn general cross-modal representations for downstream tasks. The common approach can be summarized as follows: first, the raw image-text pairs are converted into single-modality embeddings. Then an elaborate network takes these embeddings as input and produces cross-modal representations. The network is pre-trained through various pre-training tasks, after which the learned cross-modal representations can be used to solve downstream V-L tasks.

%\subsection{Transformer}
%In recent years, Transformer has gained great success in various areas, especially in natural language processing. The vanilla Transformer~\cite{vaswani2017attention} utilizes an Encoder-Decoder architecture and is proposed as a sequence-to-sequence model for machine translation task. It adopts the Scaled Dot-Product Self-Attention mechanism to draw global dependencies and employs a residual connection~\cite{he2016deep} to build a deeper model. \citeauthor{dosovitskiy2020image} proposes Vision Transformer~\cite{dosovitskiy2020image}, which uses a pure Transformer for Computer Vision tasks. ViT has achieved state-of-the-art performance on multiple image recognition benchmarks, proving the effectiveness of Transformer in both Vision and Language tasks.

%\subsection{Single-Modal Pre-training}
%With the increasing of computation power and the advance of Transformer architecture, Pre-training and Fine-tuning has become the paradigm of NLP tasks. The mainstream approach is to first pre-train a model(usually with a Transformer backbone) on a large corpus and then fine-tune it on downstream tasks. Large Pre-trained Language Models~(PLM) such as BERT~\cite{devlin2018bert} and GPT~\cite{radford2018improving}, have achieved state-of-the-art results on many Natural language understanding~(NLU) and natural language generation~(NLG) tasks. On the other hand, Pre-training and Fine-tuning for image models has made several breakthroughs such as BEiT~\cite{bao2021beit} and MAE~\cite{he2021masked}.
  
%\subsection{Vision-Language Pre-training}
%Following the success of the paradigm of pre-training and fine-tuning, many have tried to apply the same stratrgy to vision-language task. Intuitively, pre-trained with a large dataset can help vision-language model overcome the lack of data in downstream task. Most existing  models use image-text pairs for pre-training. The common approach can be summarized as followed: First, we convert the raw image-text pairs into two single-modality vector representations. Then the transformed data is passed through a large network to learn cross-modal representations. The network, on the other hand, is pre-trained on a large dataset with carefully designed pre-training tasks. At last, The learned cross-modal representations are used to solve downstream vision-language tasks.

==> sec-eval.tex <==
\section{Evaluation and Datasets}\label{eval}
In this section, we will introduce some evaluation metrics on downstream tasks and some widely-used pre-training datasets.

\subsection{Evaluation}
Since evaluation metrics are related to downstream tasks, we list the downstream tasks mentioned in \ref{downstream} and their corresponding metrics in Table \ref{metrics}.



\subsection{Datasets}
There has been an increasing amount of large-scale image-text collections for vision-language pre-training. In Table \ref{datasets} we list several widely-used or recently proposed datasets.

\begin{table}
\centering
\begin{tabular}{lll}
\hline
Dataset  & Size & Reference \\
\hline
COCO       & 328,124  & \cite{lin2014microsoft}     \\
VG       & 108,077  & \cite{krishna2017visual}      \\
CC    & 3.1M  & \cite{sharma2018conceptual}     \\
SBU   & 1M  & \cite{ordonez2011im2text}     \\
LAION & 400M & \href{https://laion.ai/laion-400-open-dataset/}{https://laion.ai/laion-400-open-dataset/} \\ 
RedCaps & 12M & \cite{desai2021redcaps} \\

\hline
\end{tabular}
\caption{Widely Used Pre-training Datasets}
\label{datasets}
\end{table}

==> sec-extensions.tex <==
\section{Extensions of VLP}\label{extensions}
V-L PTM has made significant progress over existing methods, but it can still be improved in different ways. In this section, we give a different aspect of V-L PTMs and introduce several recent breakthroughs in different areas.

\paratitle{Multi-task Learning.} Multi-task Learning(MTL) requires a single model to solve multiple tasks at the same time. Considering the significant overlap between different vision-language tasks, there is a huge potential of MTL for V-L PTMs. \citeauthor{lu202012} develops a large-scale multi-task model that is capable of dealing with 12 different tasks by learning shared trunk parameters and a set of task-specific layers for different tasks. UniT\cite{hu2021unit} utilizes an encoder-decoder architecture and uses a shared decoder to make predictions on each task over the encoded input representations. Both methods achieve strong results on corresponding downstream tasks with fewer parameters to optimize.


\paratitle{Stage-wise Pre-training.} Stage-wise Pre-training aims to break down the pre-training process into several sub-processes and complete them stage-by-stage. VLMo\cite{wang2021vlmo} uses this strategy to leverage large-scale image-only and text-only data as an augmentation for the V-L PTM. The process is achieved by pre-training different modules of the V-L PTM on corresponding data while freezing other parts(\emph{i.e.} pre-train the attention module and vision expert on image-only data) to learn a more general representation. FLAVA\cite{singh2021flava} achieves the same goal by pre-training different encoders instead of different experts. Both models show better performance compared to traditional pre-training strategies and have a stronger ability to handle unimodal data.

\paratitle{Advanced Fine-tuning Method.} Following the pre-training and fine-tuning paradigm, there are lots of methods that can be transferred from PLM to V-L PTM. CLIP-adapter\cite{gao2021clip} adopts an additional bottleneck layer to CLIP for features learning. As a consequence, CLIP-Adapter improves the performance of CLIP on few-shot setting with only a little change on model architecture. Prompt-Tuning method has also been adapted to V-L PTMs. \cite{zhou2021learning} proposes a context optimization(CoOp) method to automate prompt engineering to allow
more efficient and task-specific transfer for pre-trained vision-language models. Frozen\cite{tsimpoukelli2021multimodal} uses prompt method to fill the gap between vision and language representation. Both methods achieve success under few-shot setting.



==> sec-inputrep.tex <==
\section{MultiModal Input Representation}\label{inputrep}
As discussed in section~\ref{intro}, encoding images and texts as embeddings preserving input semantics is the first step to pre-train a V-L PTM. The way of encoding images and texts are quite different because of the discrepancy between the two modalities. In what follows, we introduce several methods to encode the images and texts into single-modal embeddings before feeding them into cross-modal transformer.

\subsection{Data Formulation}

\subsection{Text Representation}
Most existing works on V-L PTM encode text using the same technique as BERT~\cite{devlin2018bert}. A given sentence is first split into a sequence of tokens by WordPiece tokenizer~\cite{wu2016google}, generating the input word embedding sequence $W=\langle  w_1,...,w_j,...,w_n \rangle$. \textcolor{blue}{A positional embedding and a segment embedding are used to encode position information and indicate index of the word’s sentence if multiple exists.
The final input text representation is $\langle  \hat{w}_1,...,\hat{w}_j,...,\hat{w}_n \rangle$. For each of the final representation at position i, it is conculated as:
\begin{equation}
    \hat{w} = LayerNorm(w_i + p_i +s_w)
\end{equation}
where $w_i$ indicates the original word embedding, $p_i$ indicates positional embedding at index i, $s_w$ indicates index of word's sentence and LayerNorm indicates the same normalization function as BERT.
}

\subsection{Image Representation}
Since the embeddings of an image will be fed into a transformer-based architecture along with the embeddings of its paired text, most of researches represent the image as a sequence of embedding vectors: $V=\langle v_{[IMG]}, v_1, ...v_j, ...v_m\rangle$ first. In this way, we can unify input representation as sequence of embeddings for both modalities. Although there is some consensus on how text should be encoded, the way to encode an image is still evolving. We divide the way of encoding an image into three categories based on how the image feature sequence is produced.


\subsubsection{Region Features}
Most previous work uses region-based feature to give an object-level input image representation, which requires an extra object detector~(OD) to extract visual features. Each region represent an object detected from an image, which is later formed as a sequence to give an image representation. ViLBERT~\cite{lu2019vilbert} and LXMERT~\cite{tan2019lxmert} first use Faster R-CNN~\cite{ren2015faster} to extract Region-Of-Interest~(ROI) features and encode spatial position information via constructing vector from region position coordinates. 
Unicoder-VL~\cite{li2020unicoder} uses a fully-connected layer to project the ROI features and region coordinates into the same embedding space.
%Although the region-based method is intuitive and effective, the extra time-consuming object detection process can be a bottleneck for V-L PTM's inference speed. Also, regarding that the OD is frozen during most of the pre-training time, it may limit the capacity of V-L PTMs and affect their performance.
\subsubsection{Grid Features}
\textcolor{blue}{Grid-based method learns from pixels to represent an image instead of using regions detected from OD. Usually, a CNN backbone is used to learn the grid features~(pixel features).}
%\citeauthor{jiang2020defense}~\shortcite{jiang2020defense} discovers that the grid features extracted from exactly the same layer of the pre-trained OD can have a comparable result against region-based methods~(using the regions from the OD's output) for VQA~\cite{antol2015vqa}.
\textcolor{blue}{Pixel-BERT~\cite{huang2020pixel} is the first work that utilizes ResNet as backbone to extract grid features.} \textcolor{blue}{SOHO~\cite{huang2021seeing} designs a visual dictionary (VD) module containing several embedding vectors to aggregate diverse visual semantic information into visual tokens. The grid feature vector's index is computed by searching the nearest embedding vector in VD. Then the nearest embedding vector is used to represent the final visual features.} 
%Compared to region-based method, grid-based method captures more visual information and enables V-L PTM to be pre-trained in an end-to-end fashion. But the grid-feature extractor can still be very heavy sometimes.
\subsubsection{Patch Features}
With the success of ViT~\cite{dosovitskiy2020image}, more and more works try to split images into patches and use the patches for later encoding. For an image $x \in \mathbf{R}^{H \times W \times C}$, it can be splited into sequences of flatten 2D patches $x \in \mathbf{R}^{N \times (P^2\dot C)}$.  where $(H, W)$ is the resolution of the original
image, $C$ is the number of channels, $(P, P)$ is the size of each image patch, and $N$
is the resulting number of patches. %Most of the existing work follows ViT to apply transformer directly to sequences of image patches.
ALBEF~\cite{li2021align} and SimVLM~\cite{wang2021simvlm} feeds patches to an ViT encoder to extract image features. ViLT~\cite{kim2021vilt} throws away the ViT encoder and \textcolor{blue}{uses simply a linear projection of patches to present image features.} 
%Pre-training without an object detector or a heavy visual embedder, ViLT can be very fast and parameter-efficient. 
%\subsection{Image-Text Representation}
%After both text and image are represented as a sequence of embeddings, most research concatenate image and text embeddings to form the image-text representation: $H^{VW}=\langle V; H^W\rangle$.
